Excitation of f-modes during mergers of spinning binary neutron star

Tidal effects have important imprints on gravitational waves (GWs) emitted during the final stage of the coalescence of binaries that involve neutron stars (NSs). Dynamical tides can be significant when NS oscillations become resonant with orbital motion; understanding this process is important for accurately modeling GW emission from these binaries, and for extracting NS information from GW data. In this paper, we carry out a systematic study on the tidal excitation of fundamental modes of spinning NSs in coalescencing binaries, focusing on the case when the NS spin is anti-aligned with the orbital angular momentum-where the tidal resonance is most likely to take place. We first expand NS oscillations into stellar eigen-modes, and then obtain a Hamiltonian that governs the tidally coupled orbit-mode evolution. We next find a new approximation that can lead to analytic expressions of tidal excitations to a high accuracy, and are valid in all regimes of the binary evolution: adiabatic, resonant, and post-resonance. Using the method of osculating orbits, we obtain semi-analytic approximations to the orbital evolution and GW emission; their agreements with numerical results give us confidence in on our understanding of the system's dynamics. In particular, we recover both the averaged post-resonance evolution, which differs from the pre-resonance point-particle orbit by shifts in orbital energy and angular momentum, as well as instantaneous perturbations driven by the tidal motion. Finally, we use the Fisher matrix technique to study the effect of dynamical tides on parameter estimation. We find that the dynamical tides may potentially provide an additional channel to study the physics of NSs. The method presented in this paper is generic and not restricted to f mode; it can also be applied to other types of tide.

==> reply.tex <==
Dear Jocelyn,

We would like to thank you for the insightful report. Below we provide a detailed breakdown of your report, responding to each point raised. For ease of reading, we have included below the original report (commented out), and immediately below each point, we provide our response.

With kind regards,
Sizheng Ma
Hang Yu
Yanbei Chen


%Broadly this is a nice piece of work exploring semi-analytic modeling of tidal resonances. Clarity could be improved.

Reply: 

In Sec. I (Introduction) and Sec. VI (Conclusions and discussion), we added more sentences about our primary focus: To study the qualitative features of dynamical tide (DT), and to explore their semi-analytic modelings. The impacts of DT on real observations are not our main purpose yet. Therefore, in this paper we mainly focus on the cases where tidal features are the strongest, i.e., f-mode in the rapidly spinning NSs, and H4 EoS, even though they are disfavored by current detections.


%First - Several notes are left in from the authors suggesting this is not a final document. Please note if any major changes are made.

Reply:

We cleaned up all notes.

%I was surprised not to see reference to the LVC measurements of tidal effects for GW170817 (source properties or most recently the catalog paper for tidal parameter). The EOS references do not include LVC radios/EOS constraint paper 1805.11581 or model selection paper 1908.01012 (or more recent work). Also, I might expect a mention of the LVC observation of GW190425 (which is recent but public, and now accepted).

Reply:

We mentioned these references in the first paragraph of Sec. I (Introduction).

%In particular, the H4 EOS that is used as a comparison in this work is strongly disfavored compared to more compact EOS by LVC observations (see above results in particular fig 2 & 3 of https://arxiv.org/abs/1908.01012 ). This should be commented on in justifying the relevance of the results shown.

Reply:

We added sentences in Sec. II A that our paper is mainly about the qualitative features of DT. To make the effect more pronounced, we choose a stiff EoS, even though it is disfavored. We also mentioned (p6) that the general features presented in our paper don't quite depend on EoS. So our results should also be valid for other EoS.

%Also, as the authors focus on spin frequencies of 550Hz for some comparisons, it would be useful to put this in context by noting more clearly how results would apply to currently measured spins (in particular accuracy of model and comparisions with H+16 in Sec IV)in particular the observed spins of NS observed in GW (GW170817 has most likely effective spin of ~0, GW190425 https://dcc.ligo.org/P190425/public which has under the broad prior a most likely effective spin of about twice that of J1946+2052, upper bound on effective spin for both GW190425 and GW170817 translates to I think about half that of PSR J1748?2446ad.)

Reply:

We mentioned that H+16 is enough for current detections since recent events are consistent with low spin configurations. However, rapidly spinning NSs in binaries are still physically allowed. Therefore, an accurate GW model for these systems are still necessary.

%Are references to LIGO instruments/results up to date? See above for LVC results on measured properties of NS. In Sec V, please specifically link each curve used to a reference rather than citing in bulk. I think https://arxiv.org/abs/1304.0670 may be relevant? How is ligo-t1600119 used?

%late stage of inspiral for NS mergers in the LVC context is generally not 10s-100s of Hz but 100s-1000s of Hz

%I wouldn't consider dynamical tide work to be notably "preliminary" compared to adiabatic tide work, considering the last ~5 years of publications? This work seems comparable in sophistication (although with meaningful improvement) to F+07 and H+16.

Reply:

Modifications were made.

%p6 Clarify assumptions (incompressibility/Maclaurin spheroid) earlier. Comment more clearly on effectiveness of method even though (as noted) it gives unrealistic Love numbers.

Reply:

On p6, we added sentences about the validity of our assumption (Maclaurin spheroid): The equations of motion are generic, EoS affects only the values of the coupling constants, $\lambda_0$ and $\lambda_2$. Therefore, we replaced their values with those from H4 and polytrope EoSs.

%Clarify the distinction betwen the assumptions of eqs 26 and those going into the results of III.B. In general, the use of numerical is not always clear (especially as in the field it often refers to full numerical relativity)

Reply:

On p8, we clarified that results in Sec. III B are only the analytic solutions to eqs 26. Although it's straightforward to integrate them to get solutions, analytic expressions can provide us with more physical insights. 

To avoid confusion, we use numerical integrations to refer to numerical solutions. 

%I might have expected [65] to be cited much earlier in motivating this work. Possibly in the context of other numerical simulation work besides that single reference.

We moved it to Sec. I.

